Order-optimal Joint Transmission and Identification in Massive Multi-User MIMO via Group Testing

The number of wireless devices which are connected to a single Wireless Local Area Network continues to grow each year. As a result, the orchestration of so many devices becomes a daunting, resource--consuming task, especially when the resources available at the single access point are limited, and it is hard to anticipate which devices will request access at any given time. On the other hand, the number of antennas on both the devices and the access point grows as well, facilitating advanced joint scheduling and coding techniques. In this paper, we leverage the large number of antennas and suggest a massive multiple-user multiple-input-multiple-output (MU-MIMO) scheme using sparse coding based on Group Testing (GT) principles. The scheme allows for a small subset of devices to transmit simultaneously, without a preceding scheduling phase or coordination, thus reducing overhead and complexity. Specifically, we show that out of a population of \(N\) devices, it is possible to jointly identify and decode \(K\) devices, unknown in advance, simultaneously and without any scheduling. The scheme utilizes minimal knowledge of channel state, uses an efficient (in both run-time and space) decoding algorithm, and requires \(O(K\log N\mathcal{M})\) antennas, where \(\mathcal{M}\) is the number of messages per device. In fact, we prove that this scheme is order--optimal in the number of users and messages. This is done by deriving sufficient conditions for a vanishing error probability (a direct result), bounding the minimal number of antennas necessary for any such scheme (a converse result), and showing that these results are asymptotically tight.

==> TexFiles/01 - Intro/Intro.tex <==
Modern wireless communication systems have multiple antennas to increase reception and transmission quality without increasing other system resources (such as power or bandwidth).
These systems, named Multiple-Input-Multiple-Output (MIMO) systems, have become ubiquitous.
They are integrated into Cellular phones, Cellular Base Stations, IoT devices, WiFi, and many more.
Recent years re-introduced the antennas' role in MIMO systems; they can be used as an additional source of information in addition to transmitting signals into the air (a technique dubbed "Index Modulation", \cite[Chapter~1.2]{IndexModBook}).
I.e., end-points can utilize several techniques to selectively active some antenna at the receiver.
The selected antenna's index is a piece of additional information (to the sent signal) sent by the terminal.
This idea may allow multiple users to transmit simultaneously.
Still, there is a limit to the number of users that can transmit simultaneously (due to large decoding times), and a resource-sharing mechanism that distributes resources such as time, frequency bands, and code, between the users, is essential.

In large wireless networks, each end-point may interfere with the transmission of the other users via collisions.
Common approaches to the problem include medium access protocols (e.g., CSMA) or clever collision resolution algorithms such as the Capetanakis Collision-Resolution Algorithm (CCRA) or its modified version (MCCRA) in \cite[Chapter~4.2]{longo1981multi}.
When dealing with MIMO systems, we add more degrees of freedom but with increased complexity.
If the system is not well-designed (in terms of separable transmissions), each user equipped with multiple antennas may interfere with its transmissions.
A common approach to solve the interferences and collisions problem, better known as the Multiple Access Channel (MAC) problem, is scheduling, where all users agree that a relatively low number of users transmit simultaneously.
Medium access protocols or collision resolution algorithms may become obsolete when introducing user scheduling to the system, but optimal user scheduling might be infeasible.

The scheduling, or resource allocation, can be performed by a single controller (centralized control) or distributively by the users.
In centralized scheduling schemes, the controller (typically an access point or a base station) needs to distribute the resources between the users in a manner that optimizes a well-defined criterion (such as maximizing the overall rate, achieving a certain level of fairness with respect to a predefined fairness metric, etc.).
When the number of users becomes large, centralized scheduling algorithms that optimize such criteria can become intricate and do not scale well.
Accordingly, centralized schedulers typically utilize approximation algorithms.
Distributed scheduling utilizes medium access control techniques to coordinate between the users.
Such approaches can result in a failed transmission due to miscoordination.
Both approaches encompass challenges, especially when users and antennas proliferate.
On the other hand, this growth provides opportunities to devise new scheduling techniques.

Many works suggested approximation algorithms for scheduling.
The scheduling algorithms are based on channel information and user independence (such as \cite{susPaper}) or Signal-to-Noise Ratio (SNR) like in \cite{ergodicCapacity}.
These approximations are remarkably easy to implement in software (a vital point when scheduling users in 5G networks).
However, some recent works tried to solve the MAC problems using clever coding techniques (e.g., Non-Orthogonal Multiple Access, NOMA), shifting the solutions to almost hardware-level.
While NOMA allows multiple users to send information simultaneously, the number of active users at a time is greatly limited \cite{NOMA}.

Recent works use codes and algorithms originated in Group Testing (GT) to allow the joint decoding of many messages using a simple and local decoding algorithm.
GT is a technique to identify a set of defective items out of a large population.
The procedure suggests that tests are performed jointly on a group of items rather than conducting individual tests on each item.
In the communication context, the group test is replaced by a set of users transmitting simultaneously.
The GT-based solutions (like \cite{SecureGroupTesting, robin2021sparse}) combine mini-timeslots as bit times (or different frequency bands) and energy detection.
This approach is extraordinarily more efficient in local resources at the receiver - it requires only the knowledge of the codebook and a simple energy detection scheme like in \cite{enrgyDetectMIMO}.

In our proposed scheme, each user has its unique codebook generated using methods from GT.
We assume a large wireless network where a relatively low number of users transmit simultaneously to a single receiver.
Each user is equipped with a massive number of antennas, including the receiver, making our MAC problem into a massive (in the number of antennas) Multi-User MIMO (MU-MIMO) MAC problem.
In our scheme, users aim at antennas at the receiver (similar to Index Modulation) according to their corresponding codeword in their codebook.
Our scheme targets large sensor and cellular networks with a single receiver (e.g., central controller or base station).

The mentioned works related to GT usually assume noiseless and interference-free models.
Except for \cite{robin2021capacity}, most GT-based mechanisms that considered noise assumed no correlation between the set of transmitting users and the decoding error probability.
However, such an assumption is not applicable when adapting the existing GT-based communication schemes into MU-MIMO systems, such that each receiver antenna replaces a test tube (like in our scheme).
Specifically, when a set of users is transmitting to multiple antennas, the power experienced by each receive antenna is directly correlated to the transmitting user set and their target antennas.
We derive the Bit Error Rate (BER) of our scheme, closed-form expressions for Noisy Column Matching (Noisy CoMa) from \cite{CoMa}\footnote{also known as "Noisy Combinatorial Orthogonal Matching Pursuit" (N-COMP) in \cite{CoMa2, robin2021capacity} or the noise-tolerant of the Definitely Not Defective (DND) Algorithm in \cite{SecureGroupTesting}.} algorithm's error probability bounds and sufficient conditions for vanishing error probability (in both noisy and noiseless models).
We also formulate a necessary lower bound (converse) for vanishing error probability for our scheme.

==> TexFiles/01 - Intro/Intro_Short.tex <==
MIMO systems have become ubiquitous due to their increased reception and transmission quality, in both single and MU communications.
In MU communication, most MU-MIMO works focus on user selection (e.g., \cite{Xia2021approx_KKT_iterative, Zhang2021clusteredJointPowerOpt}) as a possible solution to the Multiple Access Channel (MAC) problem.
Even the 802.11ax standard, the state-of-the-art WiFi technology, solves the MAC problem by scheduling users to dedicated frequency bands \cite[Chapters~3.3.4-3.3.6]{gulasekaran2022wifi6}.
Traditional user selection carries a lot of overhead - complex optimization problems solved by a \emph{centralized unit}, information gathering (by message passing), and the scheduling announcement.
The announcements may use dedicated resources - reducing system resource efficiency.
Collecting and processing Channel State Information (CSI) to schedule users can be computationally hard when the number of users is large, so optimal user scheduling is infeasible.
Reducing this complexity encompasses many challenges;
Indeed, eliminating the need for CSI collection (at the receiver) and performing user scheduling while maintaining high rates and reliability requires sophisticated mechanisms.

We address these challenges by combining two seemingly unrelated ideas into a novel, order-optimal self-scheduling, identification, and decoding scheme.
We use Threshold-based Index Modulation \cite[Chapter~1.2]{IndexModBook}, where users selectively activate antennas at the receiver to provide additional information.
Then, we revisit the GT problem, capable of finding $K$ items of interest out of a large population of $N$ items \cite{GTBook}.
In GT, items are tested together rather than individually, minimizing the number of tests required to identify the $K$ items.

The set of items participating in each test can be determined \emph{a-priori} in the form of a test matrix.
After conducting all tests, the test conductor observes the result vector and uses decoding algorithms such as Chan's Noisy Column Matching (Noisy CoMa) \cite{CoMa, CoMa2}, also known as Noisy Combinatorial Orthogonal Matching Pursuit, to identify the defective items.

In the context of user scheduling and identification, the users are analogous to the population of $N$ items.
The $K$ items of interest are the self-scheduled users whose identity is unknown.
The test matrix is akin to a binary codebook.
The tests conducted are usually energy detection results on different system resources such as timeslots, frequency bands, or, as in the suggested scheme, antennas activated.

Modern literature suggests GT-originated codes to devise communication protocols capable of joint decoding many messages using a simple decoding algorithm.
For example, in \cite{robin2021sparse}, Robin and Erkip proposed an energy-efficient sensor discovery in power-constrained clustered networks.
Cohen \emph{et al.} proposed a GT-based communication protocol in \cite{EffiColl}, based on ideas from \cite[Supplementary~Materials]{SecureGroupTesting}.
Our work can be considered as extending Robin and Erkip's work in \cite{robin2021capacity}, which considered a Single-Input-Single-Output Rayleigh Fading Channel device discovery scheme.
The main idea is to reduce the continuous signal and noise models into discrete binary models, using energy detection, followed by Noisy CoMa for decoding.
\cite{robin2021capacity} provides a good solution in terms of reduced hardware costs due to the lack of CSI, but fails to enjoy the array gain (SNR increase), diversity gain (reduction in symbol detection error probability), or multiplexing gain (rate increase) when adding more antennas to all parties.

In the suggested scheme, users have a codebook generated using methods from GT.
The users leverage their massive number of antennas to null their transmitted signals' energy in the antennas corresponding to zeros in their allocated codeword.
Any other antenna may read some energy.
The receiver uses energy detection, converting channel output to a binary vector, to estimate which antenna is targeted by at least one user.
The binary vector is treated as the result vector of GT and is the input to a decoding algorithm which returns the sent messages (consequently, the identities of the transmitting users as well).

Our scheme requires no scheduling overhead (headers, control messages, CSI collection at the receiver, etc.) and has extraordinarily low complexity;
The number of antennas is linear in codeword length, the detectors in each antenna are simple energy detectors, and the decoding algorithm is efficient in both run-time and space.
Only the (complete) codebook is vital for its operation.
We analyze the error probability of the scheme, find a lower bound and scaling laws of the number of antennas, and show that it is order-optimal in codebook size (either in the number of users or the number of messages per user).

==> TexFiles/02 - Related Work/RelatedWork_GT.tex <==
The GT problem revolves around finding $K$ items of interest, also known as the defective items, out of a large population of $N$ items using as few as possible tests (\cite{GTBook}).
In the Non-Adaptive GT (NAGT), the set of items participating in each test is determined \emph{a-priori}.
After conducting all tests, the test conductor observes the Result Vector and identifies the defective items accordingly.

The order of tests, or equivalently when each item is tested in which group-test, forms a matrix (dubbed as the "test matrix" or "test design") whose columns represent the items and rows represent tests.
A component in the matrix is either zero (the corresponding item does not participate in the group test) or one.
The test design is either a random matrix (typically with i.i.d. Bernoulli entries like in random coding schemes. Better known as "random design") or a deterministic matrix with special intersection properties (between the test designs' rows, columns, or both) known as "block design", \cite{du2000combinatorial}.
In most cases, the desired intersections have the particular property of a constant number of items per intersection, inducing a constant weight matrix.
Block Designs are considered better than random designs (\cite{GTBook, BerCap}) in terms of the number of required tests for vanishing error probability of the separating algorithm but are much harder to find (especially when $N$ and $K$ are large, which is the case GT was designed in the first place).
There are, however, some explicit constructions of deterministic matrices with a constant number of intersections between columns.
For example, Inan et al. constructed a test design with maximal weight constraint using the Kautz-Singleton construction in \cite{sparseGT4MAC}.
The Result Vector is, essentially, the Boolean sum (Logic OR operation) of the columns corresponding to the defective items.
It is the input to an algorithm capable of \emph{separating} the columns and obtaining their indices in the test design.

Finding block designs is hard, so most GT-related works have extensively researched the random designs and the relationship between $K$, $N$, and $T$, the number of tests required for vanishing error probability of the separating algorithm.
In \cite{gtSchemeAsChannel, gtSchemeAsChannelCorrection}, Atia et al. showed a lower bound, $T = \Omega(K\log N)$ and analyzed the Maximum Likelihood Algorithm's performance resulting in $T = \Theta(K\log N)$.
Their analysis used a random Bernoulli design with parameter $1/K$.
This parameter was later fine-tuned by Aldridge et al. in \cite{ln2opt} to $p=1-2^{-1/K}$ for better separation properties.
In other words, if this parameter is used to generate the test design, the Result Vector of each $K$ columns would be unique with high probability.
For a large $K$, one can use $p=\frac{\ln 2}{K}$ as an approximation, \cite{SecureGroupTesting}.

GT's optimality lies with the growth of $K$ compared to $N$.
Agarwal et al. (\cite{impossibilityRes}) studied the linear sparsity region, where $K=\Theta(n)$, and showed that when $K\geq 0.347N$ individual testing in NAGT is, in fact, optimal.
For dense regions, $K=O(N^a)$ for $0.5\leq a\leq 1$, Scarlett et al. showed that Noisy GT could be solved with $O(K\log N)$ tests with a simple order-optimal algorithm named "Definitely Defective" (and its noise-tolerant version) in \cite{allChanDirectConverse}.
For sparser regions, many works showed order-optimal solutions like CoMa (\cite{CoMa, CoMa2}), GROTESQUE (\cite{GROTESQUE}), SAFFRON (\cite{SAFFRON}), Belief Propagation (\cite{beliefProp}) and Bit Mix Coding (\cite{BitMixCoding}).

The GT model encompasses two versions, the noise-free model and the noisy model.
The noisy version considers that test results can be corrupted by noise or dilution - a bit may flip or be erased.
Both versions (noiseless and noisy GT) were reduced into a communication system by Atia et al. in \cite{NoisyGT}.
In Atia's communication model, the set of items is analogous to the different users.
The defective items are the set of transmitting users.
The codebook is the test matrix (each column is a codeword), and the channel sums transmissions using Boolean sum.

Since GT deals with Boolean vectors, all discrete (memoryless) binary channels have been addressed in the literature.
In their later work, \cite{gtSchemeAsChannel}, Atia et al. solved the GT problem for Reversed-Z Channel (RZ-Channel) and Z-Channel.
Chan et al. addressed the Binary Symmetric Channel (BSC) in \cite{CoMa, CoMa2} and solved the GT problem using Noisy Column Matching (Noisy CoMa) from \cite{CoMa}\footnote{also known as "Noisy Combinatorial Orthogonal Matching Pursuit" (N-COMP) in \cite{CoMa2, robin2021capacity} or the noise-tolerant of the Definitely Not Defective (DND) Algorithm in \cite{SecureGroupTesting}.}.
The Binary Asymmetric Channel (BAC) was addressed by Scarlett et al. in \cite{allChanDirectConverse} and Sejdinovic et al. in \cite{beliefProp}.

Robin et al. have recently proposed using GT coding for energy-efficient sensor discovery in \cite{robin2021sparse}.
Their model assumed a noiseless channel, with a sensor network clustered to $M$ fixed-sized clusters (a widespread assumption for IoT devices).
They have studied the impact of the sensors' activity (either a fixed deterministic number is active or random activity).
They described how the sensors could simultaneously transmit to a single Access Point in their cluster.
The main idea was to use energy detection over $T$ \emph{probes} (either time slots or different frequency bands).
They used CoMa as their decoding algorithm and analyzed its error probability to identify the correct sensors.
Additionally, they have calculated the optimal CoMa fine-tuning parameters for their model.

Cohen et al. introduced security concepts to the noiseless GT problem in \cite{SecureGroupTesting} (where an eavesdropper perceives a Binary Erasure Channel with parameter $\delta$) and presented a TDMA-based protocol in \cite{EffiColl}.
They have proved that the number of tests required for both strong secrecy and reliability is $\Theta(\frac{K\log N}{1-\delta})$.
They also showed that CoMa could be used as a decoding algorithm to their scheme \emph{without any changes}.
The security is provided by the codebook and the noise of the eavesdropper.
\cite[Supplementary~Materials]{SecureGroupTesting} was the initium for \cite{EffiColl}, where Cohen extended the GT-based communication from device discovery to a block code with $M$ words for each user (a pivotal point in their secrecy proofs).

In \cite{robin2021capacity}, Robin et al. have considered a Single-Input-Single-Output (SISO) Rayleigh Fading Channel.
The main idea of their work was to reduce the continuous signal and noise models into discrete binary models using energy detection.
They have presented a thorough analysis (including codebook generation, transmission scheme, channel effects, and receiver scheme) of GT achievability in continuous models, emphasizing the low SNR region.
Our work can be considered an extension of Robin's work on MIMO systems.

==> TexFiles/02 - Related Work/RelatedWork_GT_Short.tex <==
The GT problem revolves around finding $K$ items of interest, also known as the defective items, out of a large population of $N$ items using as few as possible tests (\cite{GTBook}).
In the Non-Adaptive GT, the set of items participating in each test is determined \emph{a-priori}.
After conducting all tests, the test conductor observes the Result Vector and identifies the defective items accordingly.

The order of tests, or equivalently when each item is tested in which group-test, forms a matrix (dubbed as the "test matrix" or "test design") whose columns represent the items and rows represent tests.
A component in the matrix is either zero (the corresponding item does not participate in the group test) or one.
The Result Vector is, essentially, the Boolean sum (Logic OR operation) of the columns corresponding to the defective items.
It is the input to an algorithm capable of \emph{separating} the columns and obtaining their indices in the test design.

Most GT-related works have extensively researched the relationship between $K$, $N$, and the number of tests, $T$.
Notably, Atia et al. showed that $T = \Theta(K\log N)$ is sufficient to find the $K$ items (with arbitrarily small error probability)  using Maximum Likelihood in \cite{gtSchemeAsChannel, gtSchemeAsChannelCorrection}.
Atia has reduced the GT problem into a communication system in \cite{NoisyGT}.
In Atia's communication model, the set of items is analogous to transmitting users.
The defective items are the set of transmitting users.
The codebook is the test matrix (each column is a codeword), and the channel sums transmissions using Boolean sum.
Since GT deals with Boolean vectors, all discrete (memoryless) binary channels have been addressed in the literature.
In their later work, \cite{gtSchemeAsChannel}, Atia et al. solved the GT problem for Reversed-Z Channel (RZ-Channel) and Z-Channel.
Chan et al. addressed the Binary Symmetric Channel (BSC) in \cite{CoMa, CoMa2} and solved the GT problem using Noisy Column Matching (Noisy CoMa) from \cite{CoMa}\footnote{also known as "Noisy Combinatorial Orthogonal Matching Pursuit" (N-COMP) in \cite{CoMa2, robin2021capacity} or the noise-tolerant of the Definitely Not Defective (DND) Algorithm in \cite{SecureGroupTesting}.}.
The Binary Asymmetric Channel (BAC) was addressed by Scarlett et al. in \cite{allChanDirectConverse} and Sejdinovic et al. in \cite{beliefProp}.

Modern literature on GT engages in devising communication protocols using the same reduction, modified for well-known communication models.
For example, Robin et al. recently proposed an energy-efficient sensor discovery in power-constrained clustered networks in \cite{robin2021sparse}.
Their work used a random test design from GT with the decoding algorithm from \cite{CoMa2}.
Cohen et al. introduced Physical Layer Security concepts to the noiseless GT problem in \cite{SecureGroupTesting} (where an eavesdropper perceives a Binary Erasure Channel with parameter $\delta$) and presented a TDMA-based protocol in \cite{EffiColl}.
\cite[Supplementary~Materials]{SecureGroupTesting} was the starter for \cite{EffiColl}, where Cohen extended the GT-based communication from device discovery to a block code with $M$ words for each user (a pivotal point in their secrecy proofs).
In \cite{robin2021capacity}, Robin et al. have considered a Single-Input-Single-Output (SISO) Rayleigh Fading Channel.
The main idea of their work was to reduce the continuous signal and noise models into discrete binary models using energy detection.
Our work can be considered an extension of Robin's work for MIMO systems.

==> TexFiles/02 - Related Work/RelatedWork_MIMO.tex <==
Most of the models for wireless channels are time-shifted Affine Transformations.
The transmitted signal suffers from multiplicative noise (attenuation or fading) and additive noise, typically Additive White Gaussian Noise (AWGN).
The MIMO model extends these models by adding more antennas at the receiver and transmitter.
These additions enable transmitting multi-dimensional symbols, but at the cost of possible interferences at the receiver.
In this case, the attenuation parameter is replaced with a matrix (dubbed the channel matrix), and the noise becomes a noise vector.

Wireless systems tend to have power constraints, so it is relatively common to normalize the power constraint into units of the noise variance.
When normalized, the additive noise is modeled after the standard Gaussian Random Variable.
Furthermore, most of the analytical works on MIMO models assume each entry in the channel matrix is a \emph{Complex} Gaussian random variable, \cite[Chapter~10]{goldsmith_2005}.
Since the fading and additive noise are statistically independent, the channel variance becomes a factor in the transmitted power, so classic MIMO literature assumes a unit variance Complex Gaussians.

When multiple users transmit simultaneously, the transmitted signals of the users are mixed, resulting in a sum of affine transformations.
In MU-SISO, if the system is designed for this purpose, the receiver can decode the transmissions jointly (e.g., using GT codes like in \cite{robin2021sparse}) or successively (like NOMA).
These solutions are possible as each transmitted signal only interferes with the transmissions of other users.
The decoder can be further optimized when the distributions of attenuation and noise are known, \cite[Chapter~4]{Proakis2007}.
If the system is not designed for simultaneous transmissions, a collision occurs, and the system must run some collision resolution algorithm to recover the transmitted messages or symbols.

However, this is not the case in MU-MIMO due to the nature of matrix multiplication.
Each component after the matrix multiplication is a linear combination of the components in the originally transmitted signal.
In other words, each user is exposed to self-interference.
A technique to correlate the transmitted signals, also known as \emph{beamforming}, is required to avoid self-interference.
Mathematically, beamforming is the act of weighting the amplitude and phase of the symbols (at both ends of the communication system) according to the channel matrix or other desired properties (e.g., maximizing SNR), \cite[Chapter~5]{tse_book}.
The weights are normalized, making them akin to rotation operators.
Beamforming at the transmitter is often referred to as \emph{precoding}, whereas beamforming at the receiver is called \emph{shaping} (\cite[Chapter~10]{goldsmith_2005}).

Works related to MU-MIMO systems focus on user scheduling and analysis of the Ergodic Capacity (the average of the maximal rate based only on channel realizations) in different schemes.
\cite{susPaper} and \cite{ergodicCapacity} are examples of such works.
Particularly \cite{capMAC} uses a threshold-based scheduling algorithm on the energy detected at the antenna in a Multiple-Input-Single-Output (MISO) system.
This approach can easily fit into the GT problem with antennas as the test tubes (either energy is above the threshold or not).
The ideas from GT can eliminate the need for these scheduling schemes, reducing the complexity of MIMO systems.

Recent work by Bicais et al. in \cite{enrgyDetectMIMO} suggested using energy detection in MIMO systems for sub-Terra Hertz bands, using On-Off Keying (OOK).
Their work covered communication from one antenna to its parallel in the receiver and can be extended easily for any pair of antennas.
They also analyzed correlated channels and suggested a joint demodulation algorithm to overcome channel interferences.
Bicais' idea has used Paquelet's original idea in \cite{enrgyDetectSISO} but for multiple antennas.
Paquelet showed that the energy detection scheme is optimal when using OOK, in addition to its low complexity.

However, both \cite{enrgyDetectSISO} and \cite{enrgyDetectMIMO} do not address the MU-MIMO problem with their solutions.
The optimal thresholds derived were optimal per pair of antennas (one at the transmitter and one at the receiver).
Also, the optimal thresholds are based on side information (channel state) at the receiver;
In other words, their solution does not scale well when the number of users grows.
Furthermore, their approach might not work well when different users target the same antenna.
Each user may have a different optimal threshold, so careful user-to-antenna assignment (alternatively, scheduling) is essential.

It is possible to extend Robin's work in \cite{robin2021sparse} to MIMO systems; however, neither party (the access points or sensors) has channel state information (CSI).
On the one hand, the lack of CSI significantly reduces hardware costs.
Yet, both parties cannot enjoy the array gain (increase in SNR), diversity gain (reduction in symbol detection error probability), or multiplexing gain (rate increase) from using multiple antennas.
Additionally, they cannot use MIMO to parallelize data streams without CSI (a pivotal point in using the antennas as test tubes).

==> TexFiles/02 - Related Work/RelatedWork_MIMO_Short.tex <==
Most of the models for wireless channels are time-shifted Affine Transformations.
The transmitted signal suffers from multiplicative noise (attenuation or fading) and additive noise.
The MIMO model extends these models by adding more antennas at the receiver and transmitter.
These additions enable transmitting multi-dimensional symbols, but at the cost of possible interferences at the receiver.
In this case, the attenuation parameter is replaced with a matrix (dubbed the channel matrix), and the noise becomes a noise vector.

When multiple users transmit simultaneously, the transmitted signals of the users are mixed, resulting in a sum of affine transformations.
In MU-SISO, if the system is designed for this purpose, the receiver can decode the transmissions jointly (e.g., using GT codes like in \cite{robin2021sparse}) or successively (like NOMA).
These solutions are possible as each transmitted signal only interferes with the transmissions of other users.
The decoder can be further optimized when the distributions of attenuation and noise are known, \cite[Chapter~4]{Proakis2007}.

Works related to MU-MIMO systems focus on user scheduling and analysis of the Ergodic Capacity (the average of the maximal rate based only on channel realizations) in different schemes.
\cite{susPaper} and \cite{ergodicCapacity} are examples of such works.
Particularly \cite{capMAC} uses a threshold-based scheduling algorithm on the energy detected at the antenna in a Multiple-Input-Single-Output system.
This approach can easily fit into the GT problem with antennas as the test tubes (either energy is above the threshold or not).
The ideas from GT can eliminate the need for these scheduling schemes, reducing the complexity of MIMO systems.

Recent work by Bicais et al. in \cite{enrgyDetectMIMO} suggested using energy detection in MIMO systems for sub-Terra Hertz bands, using On-Off Keying (OOK).
Their work covered communication from one antenna to its parallel in the receiver and can be extended easily for any pair of antennas.
Bicais' idea has used Paquelet's original idea in \cite{enrgyDetectSISO} but for multiple antennas.
Paquelet showed that the energy detection scheme is optimal when using OOK, in addition to its low complexity.
However, both works do not address the multi-user problem with their solutions.
The optimal thresholds derived were optimal per pair of antennas (one at the transmitter and one at the receiver) utilizing the receiver's channel state information (CSI).
Each user may have a different optimal threshold, so careful user-to-antenna assignment (alternatively, scheduling) is essential.
Hence, their solutions are unscalable without the use of proper coding.
Using GT coding, as we suggest, extends Bicais' work to multi-user settings.

==> TexFiles/03 - Model/Model_Short.tex <==
We assume a time-slotted network of $N$ users where $K\ll N$ of them simultaneously transmit to a single receiver.
In each time slot, a different set of $K$ users may transmit, and their identity is unknown a-priory.
Every user wishes to send one out of $C$ possible messages using a \emph{single} time slot, and there is no a-priory knowledge about the distribution of which a message is sent.
The $k^{\mathrm{th}}$ user's messages are $\mathcal{W}_k = \{w_{k,1}, w_{k,2}, \dots, w_{k,C}\}$.
WLOG, the transmitting users are $[K]$, and each user wishes to transmit its first message, $w_{k,1}$.

Each transmitter has $M_t$ antennas, whereas the receiver has $M_r$ antennas.
Each transmitter has complete knowledge of its channel state at any given time but has no channel state of other transmitters (CSIT model, as named in \cite[Chapter~10]{goldsmith_2005}).
The receiver, on the other hand, has no CSI.
The channel matrix of the $k^{\mathrm{th}}$ user is $\mathbf{H}_k\in\mathbb{C}^{M_r\times M_t}$.
Each entry in $\mathbf{H}_k$ is a zero-mean Complex Gaussian Random Variable (CGRV).
We also assume a zero-mean White Complex Gaussian Additive Noise, $\underline{n}\in\mathbb{C}^{M_r\times1}$, where $[\underline{n}]_i\sim\mathcal{CN}(0, N_0)$ for all $i$.

The $k^{\mathrm{th}}$ encoder is a function that maps some $w_k\in\mathcal{W}_k$ to a complex vector $\underline{x}_k\in\mathbb{C}^{M_t\times 1}$.
The choice of $\underline{x}_k$ also depends on the CSI by utilizing beamforming (formally: $\mathcal{E}_k:\mathcal{W}_k\times\mathbb{C}^{M_r\times M_t}\to\mathbb{C}^{M_t\times 1}$).
The transmission cannot exceed some power level, $P$.
I.e., $\norm{\underline{x}_k}^2\leq P$.
For convenience, we shall assume each component of $\mathbf{H}_k$ has a unit variance\footnote{The assumption of unit variance at the channel matrix can be interpreted as the normalization of the power constraint with the fading power.
I.e., $P$ is not the transmitted power perse, but the average SNR per antenna.}, that is, $[\mathbf{H}_k]_{i,j}\sim\mathcal{CN}(0, 1)$ for all $i,j,k$.
Finally, the receiver obtains:
\small
\begin{gather}
    \label{eq:SysMod_y}
    \underline{y}
    =
    \sum_{k=1}^{K}\mathbf{H}_k\underline{x}_k + \underline{n}
\end{gather}
\normalsize

The decoder uses $\underline{y}$ to obtain the messages sent and infer the identity of the $K$ users.
(formally: $\mathcal{D}: \mathbb{C}^{M_r\times 1}\to \prod_{n=1}^N 2^{\mathcal{W}_n}\times 2^{[N]}$, where the product is the Cartesian Product).

For simplicity, $M_r = M_t$.
We assume Massive MIMO settings, so $1\ll M_t, M_r$.
When a system has a minuscule number of antennas, one can use additional time slots/frequency bands to compensate for the difference.
E.g., if our solution requires $L = l\cdot M_r$ antennas, use $l$ time slots.
In each time slot save the channel output to obtain $\{\underline{y}_i\}_{i=1}^{l}$.
Finally, $\underline{y}$ can be obtained by concatenation: $\underline{y} = (\underline{y}_1^T,\underline{y}_2^T,\dots,\underline{y}_l^T)^T$.

We are interested in the finite-block length regime, deriving different results as functions of $N$, $K$, and $C$.
$K$ is allowed to scale with $N$ (increasing the number of simultaneously transmitting users) or $C$.
We say that the system is \emph{message-user reliable} if:
\begin{align}
    \mathbb{P}(
        \mathcal{D}(\underline{y})
        &\neq
        (\underbrace{w_{1,1}, w_{2,1},\dots, w_{K,1}}_{\text{The sent messages}},
        % \underbrace{\emptyset,\dots,\emptyset}_{\substack{\text{No}\\\text{messages}}},
        \underbrace{[K]}_{\text{Identities}})
    )
    \underset{N,C\to\infty}{\xrightarrow{\hspace*{1cm}}}
    0.
\end{align}
That is, the decoder obtains \emph{exactly} $K$ messages and the correct ones.
Additionally, it must correctly identify the corresponding users.

==> TexFiles/03 - Model/Rates_Short.tex <==
Each user has $C$ codewords, meaning each user sends $\log C$ bits per transmission.
To identify the $K$ users, the receiver needs additional $\log\binom{N}{K}$ bits.
Replacing $\log\binom{N}{K}$ with its asymptotic value $K\log N$, we obtain the sum-rate of $K\log C + K\log N = K\log NC$ bits per channel use.

We are interested to compare our rate with ergodic sum-rates.
The capacity is achieved using codes in increasing block length (e.g., more time slots), whereas we use only a single time slot and a finite number of antennas.
It is, however, convenient to compare the rate with famous quantities - especially when their approximations are functions of $M_r$.
The ergodic sum-rate has been established in \cite{MIMO_MAC} (albeit for models with CSI in the receiver).
Adapting their result to our system model yields that the ergodic sum-rate with CSIT is \cite[Equation~(40)]{MIMO_MAC}:
\begin{align}
    \nonumber
    C_{Full\ CSI}
    &\approx
    M_r \cdot \mathbb{E}[
        \log (1+\rho\cdot |[\mathbf{H}_1]_{1,1}|^2)
    ]
    \\\nonumber
    &\quad
    +
    O(
        \log(1+K\cdot M_t-M_r)
    )
    \\\label{eq:ergodic_Cap_K_CSIT}
    &\leq
    M_r \cdot \log(1+\rho)
    +O(
        \log(K\cdot M_r)
    )
\end{align}
Where $\rho \triangleq \frac{P}{N_0}$.
The last transition follows Jensen's Inequality and the fact that $|[\mathbf{H}_k]_{i,j}|^2\sim\mathrm{Exp}(1)$.

For comparison, we are also interested in the settings where all users are already scheduled.
Namely, users are scheduled using Round Robin (RR).
In RR, in each time slot, \emph{exactly one} user (whose identity is well-known) transmits but may transmit at the highest rate possible.
Hence, the average ergodic Rate approximation is $\frac{K}{N}$ times the approximation for a single user given in \cite[Equation~(37)]{MIMO_MAC}:
\begin{align}
    \label{eq:ergodic_Cap_RR}
    C_{RR}
    &\approx
    \frac{K}{N}\cdot M_r\cdot\log(1+\rho)
\end{align}

==> TexFiles/04 - BER/BER_ChooseGamma.tex <==
Unlike other works related to GT, the BAC channel's parameters can be, in hindsight, selected.
This discrete channel is a direct function of $p$ (recall that $J_i$ is also a function of $p$) and $\gamma$.
Furthermore, we can transmit using any power we like as long as it meets the power constraint.
In this subsection we present different choices to pick $\gamma$ and $p$.

\subsubsection{Bit Error Minimizer}
As we introduced earlier when calculating $q_{01}$ and $q_{10}$, $\gamma$ defines a trade-off between $q_{01}$ and $q_{10}$.
We can calculate the error probability of our decision rule:
\begin{align}
    \nonumber
    p_e
    &=
    \sum_{j=0}^K \mathbb{P}(J_i = j)\cdot \mathbb{P}(\text{bit flips}|J_i = j)
    \\\nonumber
    &=
    \sum_{j=0}^K \binom{K}{j}p^j(1-p)^{K-j}\mathbb{P}(\text{bit flips}|J_i = j)
    \\\label{eq:CharaErr_AvgErrDecisionRule}
    &=
    (1-p)^K q_{01} + (1-(1-p)^K) q_{10}
\end{align}
A suitable choice of $\gamma$ can be a minimizer of the error probability per antenna, $p_e$.
I.e., the solution to:
\begin{align}
    \begin{aligned}
        \min_{p, \gamma \in \mathbb{R}}  \quad & (1-p)^K q_{01} + (1-(1-p)^K) q_{10}
        \\
        \textrm{s.t.} \quad & 
        \begin{cases}
            0 \leq \gamma \\
            0 \leq p \leq \frac{1}{2}
        \end{cases}
    \end{aligned}
\end{align}
Notice that $p_e$'s curvature in $\gamma$ or $p$ is ambiguous.

\subsubsection{BAC Capacity Maximizer}
$q_{01}$ and $q_{10}$ define some BAC as presented in figure \ref{fig:CharaErrBAC}.
Intuitively, the capacity measures the amount of information bits received per antenna.
Maximizing this quantity minimizes the number of antennas necessary for our scheme (by theorem \ref{eq:ConverseMrBound} or corollary \ref{eq:ConverseMrBoundWithC}), so a valid choice of $\gamma$ is:
\begin{align}
    \begin{aligned}
        \max_{p, \gamma \in \mathbb{R}}  \quad & \capacity{BAC(q_{01},q_{10})}
        \\
        \textrm{s.t.} \quad & 
        \begin{cases}
            0 \leq \gamma \\
            0 \leq p \leq \frac{1}{2}
        \end{cases}
    \end{aligned}
\end{align}
We provide a contour plot of the channel capacity as a function of $\rho$ and $\gamma$ in figure \ref{fig:CharaErrBAC_contour}.
\begin{figure}[!htbp]
    \centering
    \begin{tikzpicture}[x=1pt, y=1pt, yscale=-1, xscale=1]
        % Nodes
        \node (X) at (55,72.5) {$X$};
        \node (Y) at (265,72.5) {$Y$};
        \node (0Orig) at (65,30) {$0$};
        \node (1Orig) at (65,115) {$1$};
        \node (0Chan) at (255,30) {$0$};
        \node (1Chan) at (255,115) {$1$};
        
        % Edges
        \draw[-stealth]    (0Orig) -- (0Chan) node[midway, above] {$1-q_{01}$};
        \draw[-stealth]    (1Orig) -- (1Chan)  node[midway, below] {$1-q_{10}$};
        \draw[-stealth]    (0Orig) -- (1Chan)  node[near start, below] {$q_{01}$};
        \draw[-stealth]    (1Orig) -- (0Chan) node[near start, above] {$q_{10}$};
    \end{tikzpicture}
    \caption{BAC with transition probabilities $q_{01}$ and $q_{10}$.
    When a bit is transmitted, it can flip into the other bit, and this probability depends on the transmitted bit.
    }
    \label{fig:CharaErrBAC}
\end{figure}
\begin{figure}[!htbp]
    \centering
    \includegraphics[scale=0.17]{Images/04 - BER/cBAC_300.jpg}
    \caption{
    Contour plot of the BAC capacity for $N_0 = 1$, $K = 3$ and $p = \frac{\ln 2}{K}$.
    Brighter color (closer to yellow) implies higher capacity.
    As $\rho$ increases, a lower $\gamma$ is required to get closer to one bit per antenna.
    The red line corresponds to $\gamma = \rho$, and the capacity for this choice is greatly lower than any other choice of $\gamma$.
    The curve $\gamma = \ln (\rho + 1)$ is close to the optimal choice of $\gamma$ (as it is closer than any other choice to the nearest point per contour line).
    The black curve is corresponds to $\gamma_{eq}$, the equalizer of $q_{01}$ and $q_{10}$.
    }
    \label{fig:CharaErrBAC_contour}
\end{figure}

\subsubsection{Reduction to Solved Cases}
\label{subsubsect:CoMa_reduce}
Assume we solve $q_{01} = q_{10}$ for $\gamma$ when $p = \frac{0.5}{K}$ to obtain $\gamma_{eq}$.
When using $\gamma_{eq}$, our MAC problem can be reduced to Chan et al.'s GT problem with symmetric noise (\cite{CoMa2}), so $M_r = O(K\log N)$.


==> TexFiles/04 - BER/BER_ErrProbCalc_Short.tex <==
If no additive noise exists, the result vector, $\underline{Y}$, is a Boolean Sum of the $K$ transmitted messages (when selecting $\gamma=0$).
When the additive noise is present, we have to use some mechanism to differentiate between the noise and send signals.
Since we are sampling $\underline{y}$ once, we use an energy threshold to convert $\underline{y}$ to $\underline{Y}$.
Therefore, we are interested in the following random variable:
\begin{align}
    \label{eq:CharaErr_Yi_def}
    [\underline{Y}]_i
    =
    \begin{cases}
        1 & |[\underline{y}]_i|^2 > N_0\cdot\gamma \\
        0 & |[\underline{y}]_i|^2 \leq N_0\cdot\gamma
    \end{cases}
\end{align}
$[\underline{Y}]_i$ estimates whether \emph{at least one} user targets the $i^{\mathrm{th}}$ antenna or not.
$[\underline{Y}]_i$ are i.i.d. due to symmetry.
Naturally, the estimation may err - either due to weak transmissions (caused by either deep fade or intense noise), denoted by $q_{10}$, or the additive noise overcomes the threshold when no user targets the antenna (denoted by $q_{01}$).
% We calculate both probabilities in Appendix \ref{appendix:proof_CharaErr_yi2_dist}.
Due to brevity, we present the results of the calculations in the following theorems:
\begin{theorem}
\label{eq:CharaErr_q01}
For any $\gamma$, the crossover probability from '0' to '1' is $q_{01} = e^{-\gamma}$.
\end{theorem}

\begin{theorem}
\label{eq:CharaErr_q10}
For any $\gamma$, the crossover probability from '1' to '0' is:
\begin{gather}
    \nonumber
    q_{10}
    =
    \sum_{j=1}^K \binom{K}{j}\frac{p^j(1-p)^{K-j}}{1-(1-p)^K}\bigg(1 - \exp\bigg\{-\frac{\gamma}{j \cdot \rho + 1}\bigg\}\bigg)
\end{gather}
\end{theorem}
\emph{Proof Sketch}:
We first notice that the number of users targeting an antenna, $J_i$, is Binomially distributed with parameters $K$ and $p$.
Each signal is a CGRV, and $J_i$ independent CGRVs are summed.
By using the Random Variable Transformation Theorem, we observe that the energy, conditioned on $J_i$, is exponentially distributed (with parameter $\frac{1}{J_i\cdot P + N_0}$).
Hence, $q_{01}$ and $q_{10}$ can be calculated straightforwardly to obtain the above results.
% $\rho$ can be interpreted as the SNR of the \emph{faded signal} against the additive noise, and $\gamma$ is the normalization of threshold into units of $N_0$, rather than energy.

==> TexFiles/05 - Noisy CoMa/Beta_Scale_Short.tex <==
This subsection shows different scaling laws on $\beta$ as a function of $K$ and $\rho$.
First, we shall show that $\beta$ converges to some constant term when $K\to\infty$.
\begin{lemma}
\label{lem:beta_scale_K_inf}
Let $\beta$ be the solution to the optimization problem in Theorem \ref{theo:main_result}.
Then, $\beta\to\mathrm{const.}$ when $K\to\infty$.
\end{lemma}
\emph{Proof Sketch}:
The proof will be attached in the complete version.
Recalling that $\alpha = K\cdot p$, we can invoke the Poisson Limit Theorem on $q_{10}$.
Any other term dependant on $K$ tends to some exponent powered by $\alpha$, so $\beta$ tends to some constant.

For $\beta$'s scaling with $\rho$, we observe that the expression in Theorem \ref{theo:CoMa_b_opt_prob_equiv} is not a function of $\rho$, except for $q_{10}$ (Theorem \ref{eq:CharaErr_q10}).
From this observation, we have the following (immediate) result:
\begin{corollary}
\label{lem:beta_scale_rho}
If $\rho\to0$ then $\beta\to\infty$.
If $\rho\to\infty$ then $\beta\to\mathrm{const.}$
\end{corollary}

==> TexFiles/05 - Noisy CoMa/Discussion.tex <==
% We compare our system rate in (\ref{eq:compare_our_rate}) with (\ref{eq:ergodic_Cap_K}), (\ref{eq:ergodic_Cap_K_CSIT}) and (\ref{eq:ergodic_Cap_RR}) by dividing them.
We compare our system rate in (\ref{eq:compare_our_rate}) with (\ref{eq:ergodic_Cap_K_CSIT}) and (\ref{eq:ergodic_Cap_RR}) by dividing them.
The ratios are:
\begin{align}
    % \label{eq:compare_rate_ratio}
    % \frac{C_{ergodic}}{R}
    % &\approx
    % \beta\cdot\log(\rho \cdot \beta K^2\log NC+1)
    % \\
    \label{eq:compare_rate_ratio_CSIT_only}
    \frac{C_{Full\ CSI}}{R}
    &\lessapprox
    \beta\cdot \log(1+\rho)
    +
    O\bigg(
        \frac{\log(K^2\log NC)}{K\log NC}
    \bigg)
    \\\label{eq:compare_rate_ratio_RR}
    \frac{C_{RR}}{R}
    &\approx
    \frac{K}{N}\cdot\beta\cdot\log(1+\rho)
\end{align}
We observe two kinds of losses;
The first is SNR loss, where we analyze how the rate ratios scale with $\rho$.
The other loss is the User-Codebook Loss, where we observe how the rate ratios scale with $N$, $C$, and $K\leq N\cdot C$.

When $\rho\to0$, all ratios tend to infinity by corollary \ref{lem:beta_scale_rho} below - a direct result of Shannon's Power Efficiency Limit (SPEL); it is a lower bound on the energy per bit, equivalently on $\rho$, from which onward a communication system can achieve vanishing error rates.
In the Full CSI settings, users cooperate to create dedicated virtual channels resulting in non-zero sum-rates.
Cooperation is not possible in our scheme due to the lack of irrelevant CSI.
Additionally, SPEL restricts the performance of energy detection in low SNRs.
When $\rho\to\infty$, the SNR loss scales like $O(\log\rho)$.

The User-Codebook Loss, however, scales differently.
% In (\ref{eq:compare_rate_ratio}), the User-Codebook Loss is $O(\log(K^2\log NC))$ (see how $\beta$ scales with $K$ in lemma \ref{lem:beta_scale_K_inf} below), which tends to infinity when $N C\to\infty$ and $K=O(N C)$.
In (\ref{eq:compare_rate_ratio_CSIT_only}) the loss \emph{tends to zero}, so our scheme is order-optimal when either the number of users or the number of messages grow.
The User-Codebook Loss in (\ref{eq:compare_rate_ratio_RR}) vanish when $N\to\infty$ and $K = o(N)$.
% Despite the increase in loss due to the user identity knowledge, there are scenarios where the ratio tends to zero.
I.e., if $K$ is small enough, scheduling is ineffective as it forces all users but one to idle.

==> TexFiles/05 - Noisy CoMa/NoiselessCoMa.tex <==
\improvement{More explanation of the solving scheme?}
The solving scheme is this case is random binning.
First, we generate $N\cdot C$ codewords, each is of length $\beta\log(N\cdot C)$ (where $\beta\geq1$ is some constant to be determined later).
Each bit is generated i.i.d. using Bernoulli distribution with parameter $p$.
Now we distribute $C$ codewords to each users - i.e., each user has a $C$-sized codebook.
To transmit the $m^{\mathrm{th}}$ codeword, a user selects the $m^{\mathrm{th}}$ codeword and uses ZFBF to "imitate" it on the receiver's antennas.
I.e., each user beamforms their signals such that the receiver, when calculating the component-wise $|\underline{y}|$ will read non-zero values in the corresponding locations to the $m^{\mathrm{th}}$ codeword.
In the noiseless case, ZFBF assures that if no user transmits to the $i^{\text{th}}$ receiving antenna, then the energy reading result of it will yield zero.
I.e., $[\underline{Y}]_i$, as defined in (\ref{eq:CharaErr_Yi_def}), can be translated into '1' if some energy is detected and '0' otherwise.

Decoding in the noiseless case is the vanilla GT problem - the receiver deducts the $K$ items of interest (transmitted codewords) from an uncorrupted Result Vector.
This problem has been solved in \citep{SecureGroupTesting, EffiColl}, extending \citep[Theorem~III.1]{gtSchemeAsChannel} for $C$ codewords per user rather than one.
The decoding algorithms suggested in \citep{SecureGroupTesting} are the Maximum-Likelihood decoder and CoMa.
Hence, the error probability of the scheme tends to zero if $M_r = O(K\log N C)$ and $p=\frac{\ln 2}{K}$ (\citep[Lemma~1]{EffiColl}).

==> TexFiles/05 - Noisy CoMa/NoisyCoMa_Short.tex <==
We shall follow the footsteps of \cite[Section~V.B]{CoMa}, which analyzes the Noisy CoMa algorithm for a Binary Symmetric Channel with parameter $q$.
The steps are very similar, except for the different discrete channels in which a test tube ($[\underline{Y}]_i$ in our case) is corrupt.
Our relaxation criterion will be the same as in \cite[Chapter~IV]{robin2021capacity}.

First, we consider the probability that some antenna reads '1', $p_1$.
This probability is equivalent to some component of the transmitted codeword being "hidden" by other codewords or noise.
We can calculate this probability by calculating its complement, $p_0 \triangleq \mathbb{P}([\underline{Y}]_i = 0) = (1-(1-p)^K)q_{10} + (1-p)^K (1-q_{01})$.

\begin{theorem}
\label{theo:CoMa_pMD_to0_suff_cond}
Set $M_r = \beta_1 \cdot K\log NC$.
If $\beta_1$ satisfies:
\begin{align}
    \nonumber
    \beta_1 \geq \frac{(1+\delta)\ln 2}{\alpha\big(1-\exp\big\{-2(q_{10}\Delta)^2\big\}\big)}
\end{align}
then $p_{MD}\leq (NC)^{-\delta}$ for any $\delta \geq 0$ we like.
\end{theorem}
\noindent
Likewise, we have a sufficient condition on $p_{FA}$:
\begin{theorem}
\label{theo:CoMa_pFA_to0_suff_cond}
Set $M_r = \beta_2 \cdot K\log NC$ and $\Delta < \frac{p_0}{q_{10}}-1$.
If $\beta_2$ satisfies:
\begin{align}
    \nonumber
    \beta_2\geq \frac{(1+\delta)\ln 2}{\alpha\big(1-\exp\big\{-2(p_0-q_{10}(\Delta+1))^2\big\}\big)}
\end{align}
then $p_{FA}\leq (NC)^{-\delta}$ for any desired $\delta \geq 0$.
\end{theorem}
\emph{Proof Sketch}:
We bound $p_{MD}$ ($p_{FA}$) three times (union and Hoeffding bounds followed by Taylor approximation).
Afterward, we substitute $\beta_1$ ($\beta_2$) with their respective values from the above theorems.
We will present the formal proofs in the full version, which can be found in ArXiv \cite{Vershinin2022MIMO_GT}.
% can be found in Appendices \ref{appendix:proof_CoMa_pMD_to0_suff_cond} and \ref{appendix:proof_CoMa_pFA_to0_suff_cond} respectively and are omitted due brevity.

We are interested in a vanishing error probability for our scheme, so we would like to take $\beta$ such that both $p_{MD}$ and $p_{FA}$ tend to zero.
In other words, an appropriate choice of $\beta$ is the solution to the optimization problem of minimizing the number of antennas in our scheme:
\begin{align}
    \label{eq:CoMa_b_opt_prob_orig}
    \begin{aligned}
        \min_{\Delta,\alpha,\gamma \in \mathbb{R}}  & \max\{\beta_1,
        \beta_2\}
        \\
        \textrm{s.t.} \quad & 
        0 < \Delta < \frac{p_0}{q_{10}}-1;\quad
            0 < \alpha \leq \frac{K}{2};\quad
            0 < \gamma
        % \begin{cases}
        %     0 < \Delta < \frac{p_0}{q_{10}}-1 \\
        %     0 < \alpha \leq \frac{K}{2}\\
        %     0 < \gamma 
        % \end{cases}
    \end{aligned}
\end{align}

The following theorem simplifies the optimization problem:
\begin{theorem}
\label{theo:CoMa_b_opt_prob_equiv}
The optimization problem in (\ref{eq:CoMa_b_opt_prob_orig}) is equivalent to the optimization problem in Theorem \ref{theo:main_result} and has a unique solution.
\end{theorem}
The proof is technical and will appear in the full version.
\emph{Proof Sketch}:
The proof has five steps;
(1) simplify $\Delta$'s upper bound, $\frac{p_0}{q_{10}}-1$, to $(1-p)^K\frac{1-q_{01}-q_{10}}{q_{10}}$.
(2) eliminate the dependency on $\Delta$ and convert the minimax problem into a minimization problem (by noticing that $\beta_1$ and $\beta_2$ have opposing trends in $\Delta$, so $\Delta^*$ is their equalizer).
(3) bound $\alpha^*$ to the interval $[0, e-1]$.
(4) show that for each $\alpha$ there exists a unique $\gamma^*$ minimizing the objective function.
By putting all steps together, by the continuity of the objective function, a solution exists.
Step (4) assures its uniqueness.
Finally, the final step shows that numerical algorithms will converge to $(\alpha^*, \gamma^*)$ (equivalently, $(p^*, \gamma^*)$), which is an interior point in $[0, \frac{K}{2}]\times [0,\infty)$, by putting all previous steps together and the fact that some boundary points are infeasible.

==> TexFiles/06 - Converse/Converse_Short.tex <==
In this section, we shall derive a lower bound on the number of antennas.

\begin{theorem}
\label{eq:ConverseMrBound}
Assume $N$ users, each with a $C$-sized codebook.
Assume $K$ of them wish to transmit a single codeword.
Then, a lower bound on the number of antennas, $M_r$, is required to obtain the $K$ messages reliably when using a hard-decision criterion at the receiver is:
\begin{align}
    \nonumber
    M_r \geq \frac{K\log \frac{N\cdot C}{K}}{C_{BAC} (q_{01},q_{10})}
\end{align}
Where $C_{BAC} (q_{01},q_{10})$ is the BAC capacity (\cite{BACCapacity}):
\begin{align}
    \label{eq:CharaErrCapBAC}
    &C_{BAC} (q_{01},q_{10})
    =
    \frac{q_{01}}{1-q_{01}-q_{10}}\cdot H(q_{10})
    \\\nonumber
    &\ \ \ \ -\frac{1-q_{10}}{1-q_{01}-q_{10}}\cdot H(q_{01})
    +\log\bigg( 1+2^{\frac{H(q_{01})-H(q_{10})}{1-q_{01}-q_{10})}} \bigg)
\end{align}
$H(\cdot)$ is the binary entropy function
\end{theorem}
\emph{Proof Sketch}:
The proof is similar to \cite[Chapter~IV]{CoMa2}.
Notice that the $K$ messages, their corresponding codewords, the "clean" Boolean sum, the noisy output vector, the estimated codewords, and estimated messages form a Markov Chain.
We use Fano's Inequality and Data Processing Inequality to bound the entropy of the messages and use algebraic manipulations to obtain the result.

Dividing our the converse bound with our scheme's number of antennas yields:
\begin{align}
    \frac{K\log \frac{N\cdot C}{K}}{C_{BAC} (q_{01},q_{10})}\cdot
    \frac{1}{\beta K\log NC}
    =
    \frac{1-\frac{\log K}{\log NC}}{\beta\cdot C_{BAC} (q_{01},q_{10})}
\end{align}
Which tends to a constant when $NC\to\infty$.
In other words, our scheme's number of antennas is asymptotically tight when $N$ and $C$ grow as long as $K < NC$.
According to corollary \ref{lem:beta_scale_rho}, the same claims hold when $\rho\to\infty$ and $N$, $C$ and $K$ are constant.


==> TexFiles/07 - Comparison/Compare.tex <==
In \citep[Definition~2]{MIMO_MAC}, Rhee and Cioffi defined the sum \emph{Ergodic} Capacity achievable by $K$ users under average power constraint per user and uniform power allocation (which proved to be optimal by Telatar in \citep{TelatarPaper}).
Adapting their definition to our system:
\begin{align}
    \label{eq:Ergodic_Cap_K}
    \capacity{MAC}
    =
    \mathbb{E}\bigg[
        \log\mathrm{det}\bigg(
            \mathbf{I}_{M_r} + \rho\cdot\sum_{i=1}^K \mathbf{H}_i\mathbf{H}^*_i
        \bigg)
    \bigg]
\end{align}
This quantity is hard to evaluate in software (due to overflows mid-calculation), so we will use an asymptotic approximation instead.
Using the law of large numbers like in \citep{TelatarPaper}:
\begin{align}
    \nonumber
    \lim_{M_t\to\infty} \frac{1}{M_t}\mathbf{H}_i\mathbf{H}_i^*
    =
    \mathbf{I}_{M_r}
\end{align}
Then, we have the following approximation:
\begin{align}
    \nonumber
    \capacity{MAC}
    &\approx
    \log\mathrm{det}(\mathbf{I}_{M_r} + K\cdot \rho \cdot M_t\cdot\mathbf{I}_{M_r})
    \\\nonumber
    &=
    \log\mathrm{det}((K\cdot \rho \cdot M_t+1)\cdot\mathbf{I}_{M_r})
    \\\nonumber
    &=
    M_r\cdot\log(K\cdot \rho \cdot M_t+1)
    \\\nonumber
    &=
    M_r\cdot\log(K\cdot \rho \cdot M_r+1)
\end{align}
We also compare our scheme's rate to the capacity in \citep[Equation~(40)]{MIMO_MAC} since only the transmitters have CSI and $K\cdot M_t > M_r$.
Writing the capacity explicitly:
\begin{align}
    \nonumber
    \capacity{MAC_{CSIT}}
    &\approx
    M_r \cdot \mathbb{E}[
        \log (1+\rho\cdot |[\mathbf{H}_1]_{1,1}|^2)
    ]
    \\\nonumber
    &\quad+
    O(
        \log(1+K\cdot M_t-M_r)
    )
    \\\nonumber
    &=
    M_r \cdot \mathbb{E}[
        \log (1+\rho\cdot |[\mathbf{H}_1]_{1,1}|^2)
    ]
    \\\nonumber
    &\quad+
    O(
        \log(K\cdot M_r)
    )
    \\\nonumber
    &\leq
    M_r \cdot \log(1+\rho)
    % &=
    % M_r \cdot \frac{\exp\{\rho^{-1}\}}{\ln 2}\cdot \int_{1/\rho}^{\infty}\frac{e^{-t}}{t}dt
    % \\\nonumber
    % &\quad+
    +O(
        \log(K\cdot M_r)
    )
\end{align}
The last transition follows from the fact the $|[\mathbf{H}_k]_{i,j}|^2\sim\mathrm{Exp}(1)$ for any $k,i,j$ and Jensen's Inequality.
% We define $Ei(\rho)\triangleq \int_{1/\rho}^{\infty}\frac{e^{-t}}{t}dt$ to be the exponent integral function.

In our scheme, each user has $C$ different beamforming options to send their codewords, which means each user sends $\log C$ per transmission.
From the codebook construction, the receiver also gains additional $\frac{1}{K}\log\binom{N}{K}\approx \log N$ (when $K=o(N)$) bits per user (i.e., identification without a header).
In other words, we can think of each beamforming option as a "single symbol" selection out of possible $\log (N\cdot C)$ symbols.
Hence, the sum-rate is (\citep[Corollary~1]{EffiColl}):
\begin{align}
    \nonumber
    R
    &=
    K\cdot \log C + \log\binom{N}{K}
    \\
    &\approx
    K\cdot \log (N\cdot C)
    \\
    &=
    M_r\cdot\frac{1}{\beta}
\end{align}
The ratios between the sum-rates are:
\begin{align}
    \label{eq:compare_rate_ratio}
    \frac{\capacity{MAC}}{R}
    &=
    \beta\cdot\log(K\cdot \rho \cdot M_r+1)
    \\\label{eq:compare_rate_ratio_CSIT_only}
    \frac{\capacity{MAC_{CSIT}}}{R}
    &\leq
    \beta\cdot \log(1+\rho)
    % \frac{\beta}{\ln 2}\cdot e^{\frac{1}{\rho}}\cdot Ei(\rho)
    +
    O\bigg(
        \frac{\log(K\cdot M_r)}{M_r}
    \bigg)
\end{align}
Both (\ref{eq:compare_rate_ratio}) and (\ref{eq:compare_rate_ratio_CSIT_only}) tend to infinity when $\rho\to0$ by lemma \ref{lem:beta_scale_rho}.
This is due to Shannon's Power Efficiency Limit (SPEL); it is a lower bound on the energy per bit, equivalently on $\rho$, from which onward a communication system can achieve vanishing error rates.
In the Full CSI settings, each user may cooperate with the others (including the receiver) to achieve \emph{some} non-zero rate by using dedicated virtual channels (using Singular Value Decomposition) since the receiver can perform optimal shaping.
Cooperation is possible in the complete CSIT settings (and arguably beneficial for all users as our scheme uses joint decoding).
Cooperation is not possible in our scheme due to the lack of irrelevant CSI, and SPEL restricts the performance of hard decisions on each antenna.
The restriction is evident from lemma \ref{lem:beta_scale_rho}, as $q_{10}+q_{01} = 1$ when $\rho\to 0$, so the receiver always errs resulting in zero rate.

In terms of an increasing number of users (active or not) or codewords, our scheme is order-optimal - up to a factor of $O(\log\rho)$.
%$O(e^{\frac{1}{\rho}}\cdot Ei(\rho))$.
(\ref{eq:compare_rate_ratio_CSIT_only}) can be thought of as a sum of an SNR-related Loss and a User Number-related Loss.
The User Number Loss tends to zero when $N\cdot C\to\infty$ \footnote{ this is true for $K=O(N)$ in general}, so our solution does not underperform compared to the optimal CSIT solution.
On the other hand, our system underperforms the optimal solution in the Full CSI settings due to the lack of CSI at the receiver.
The factor of the underperformance is $O(\log(K\cdot M_r))$, as $\beta$ tends to a constant from lemma \ref{lem:beta_scale_rho}.
When $\rho\to\infty$, our scheme becomes suboptimal - the SNR Loss in (\ref{eq:compare_rate_ratio_CSIT_only}) and the rate ratio in (\ref{eq:compare_rate_ratio}) tend to infinity as $\rho\to\infty$.

% Rhee and Cioffi established the sum-rate \emph{Ergodic} Capacity achievable by $K$ users in \citep[Definition~2]{MIMO_MAC}.
% Adapting their definition to our system:
% \begin{align}
%     \label{eq:Ergodic_Cap_K}
%     \capacity{MAC}
%     &=
%     \mathbb{E}\bigg[
%         \log\mathrm{det}\bigg(
%             \mathbf{I}_{M_r} + \rho\cdot\sum_{i=1}^K \mathbf{H}_i\mathbf{H}^*_i
%         \bigg)
%     \bigg]
%     \\
%     &\approx
%     \log\mathrm{det}(\mathbf{I}_{M_r} + K\cdot \rho \cdot M_t\cdot\mathbf{I}_{M_r})
%     \\
%     &=
%     M_r\cdot\log(K\cdot \rho \cdot M_r+1)
% \end{align}
% Where the approximation used the law of large numbers, similar to \citep[Equation~(6)]{TelatarPaper}.
% Notably, the sum-rate Ergodic Capacity in CSIT-only is \citep[Equation~(40)]{MIMO_MAC}:
% \begin{align}
%     \nonumber
%     \capacity{MAC_{CSIT}}
%     &\approx
%     M_r \cdot \mathbb{E}[
%         \log (1+\rho\cdot |[\mathbf{H}_1]_{1,1}|^2)
%     ]
%     \\
%     &\quad+
%     O(
%         \log(1+K\cdot M_t-M_r)
%     )
%     \\
%     &\leq
%     M_r \cdot \log(1+\rho)
%     +O(
%         \log(K\cdot M_r)
%     )
% \end{align}
% The last transition follows from the fact the $|[\mathbf{H}_k]_{i,j}|^2\sim\mathrm{Exp}(1)$ and Jensen's Inequality.

% In our scheme, each user has $C$ different beamforming options to send their codewords, which means each user sends $\log C$ per transmission.
% From the codebook construction, the receiver also gains additional $\frac{1}{K}\log\binom{NC}{K}\approx\log NC$ (when $K=o(N)$) bits per user (i.e., identification without a header).
% In other words, we can think of each beamforming option as a "single symbol" selection out of possible $\log (N\cdot C)$ symbols.
% Hence, the sum-rate is (\citep[Corollary~1]{EffiColl}):
% \begin{align}
%     \label{eq:compare_our_rate}
%     R
%     &\approx
%     K\cdot \log (N\cdot C)
%     =
%     M_r\cdot\frac{1}{\beta}
% \end{align}

==> TexFiles/07 - Comparison/Compare_Short.tex <==
This section compares our scheme's rate with the Ergodic sum-rates by calculating rate ratios.
Our rate is given in (\ref{eq:compare_our_rate}) and the Ergodic sum-rates are given in (\ref{eq:Ergodic_Cap_K}) and (\ref{eq:Ergodic_Cap_K_CSIT}).
The ratios are:
\begin{align}
    \label{eq:compare_rate_ratio}
    \frac{\capacity{MAC}}{R}
    &=
    \beta\cdot\log(K\cdot \rho \cdot M_r+1)
    \\\label{eq:compare_rate_ratio_CSIT_only}
    \frac{\capacity{MAC_{CSIT}}}{R}
    &\leq
    \beta\cdot \log(1+\rho)
    +
    O\bigg(
        \frac{\log(K\cdot M_r)}{M_r}
    \bigg)
\end{align}
Both (\ref{eq:compare_rate_ratio}) and (\ref{eq:compare_rate_ratio_CSIT_only}) tend to infinity when $\rho\to0$ by lemma \ref{lem:beta_scale_rho} - a direct result of Shannon's Power Efficiency Limit (SPEL); it is a lower bound on the energy per bit, equivalently on $\rho$, from which onward a communication system can achieve vanishing error rates.
In the optimal solutions (in both Full CSI and complete CSIT settings), users cooperate to create dedicated virtual channels resulting in non-zero sum-rates.
Cooperation is not possible in our scheme due to the lack of irrelevant CSI.
Additionally, SPEL restricts the performance of energy detection in low SNRs.

(\ref{eq:compare_rate_ratio_CSIT_only}) can be thought of as a sum of an SNR Loss and a Codebook Size Loss.
The Codebook Size Loss tends to zero when $N\cdot C\to\infty$ (for any $K$), so in terms of an increasing number of users (active or not) or codewords, our scheme is order-optimal up to a factor of $O(\log\rho)$.

==> TexFiles/08 - NumerRes/results_Short.tex <==
Figure \ref{fig:rate_ratio_N} compares the rates in Subsection \ref{subsect:Rates} with our scheme's rate.
We also compare our rate with MU systems used in practice - errorless satellite networks (using data provided by AYECKA) and oracle-aided errorless 802.11ax.
% The blue line is the ratio between the optimal solution (with Full CSI) and our scheme, given in (\ref{eq:ergodic_Cap_K}).
The blue line is (\ref{eq:ergodic_Cap_K_CSIT}), whereas the orange line is (\ref{eq:ergodic_Cap_RR}).
The yellow line is the sum-rate of our scheme, (\ref{eq:compare_our_rate}).
The purple line is the sum-rate of raw transmissions at the highest symbol rate of a $K$-to-1 satellite communication (normalized by its bandwidth).

The green line is the sum-rate of a $160$MHz 802.11ax, normalized by a single carrier's bandwidth ($78.125$kHz).
The oracle schedules the $K$ users without passing requests or scheduling information.
I.e., they do not send $\log N$ \emph{header} bits for identification.
The receiver sends a trigger frame followed by a short silent interval (named SIFS).
Afterward, the users transmit their frames simultaneously on different frequency bands.
Payload size is $\log C$ (for a fair comparison) and is sent in MCS2 rate, and the rest is according to the 802.11ax standard (one training field and $8\mu$sec packet extension).
The sum-rate also considers the trigger frame (sent in MCS0 rate) to allocate resources to the $K$ users; each is scheduled to 200 frequency bands.
The sum-rate can be further reduced when considering the $\log N$ header bits and the scheduling information.
Our scheme achieves higher sum-rates than 802.11ax (when the number of users is big enough) or satellite networks and has no significant overheads.

\begin{figure}
    \centering
    % \includegraphics[scale=0.16]{Images/08 - NumerRes/rate_ratio_N.jpg}
    \input{TexFiles/TexImages/rates_N}
    \caption{
        Different (normalized in bandwidth) rates as functions of $N$ when $\rho=20_{\mathrm{dB}}$, $K=10$, $C=1000$, $\delta=0.33$ and $N_0 = 2$.
        The 802.11ax is oracle-aided; the $K$ users are scheduled without passing information to the access point.
        The coefficient multiplying the logarithmic term in (\ref{eq:ergodic_Cap_K_CSIT}) is 1.
    }
    \label{fig:rate_ratio_N}
\end{figure}

Figure \ref{fig:spec_eff} compares our scheme's Spectral Efficiency from (\ref{eq:compare_our_spec_eff}) with SPEL, evaluated for different settings of $K$, $N$ and $C$.
The SPEL is calculated like in \cite[Chapter~3.5]{srinivasan2020wireless}.
For our system, we have used $\frac{E_b}{N_0} = \frac{K\cdot P}{N_0\cdot M_r}$.
The bold dark line is SPEL, and its dashed counterpart is the \emph{absolute} SPEL, $\ln 2$.
The purple line is the limit of $\beta^{-1}$ when $K\to\infty$ (calculated regardless of $N$ or $C$).
\begin{figure}
    \centering
    % \includegraphics[scale=0.16]{Images/08 - NumerRes/spec_eff.jpg}
    \input{TexFiles/TexImages/spec_eff}
    \caption{
        Spectral Efficiency as a function of $\rho$ (in $\mathrm{dB}$) when $\delta=0.33$ and $N_0 = 2$.
        The mentioned probabilities, $q_e\triangleq(1-p)^K q_{01} + (1-(1-p)^K) q_{10}$, are the BER of the blue line at the corresponding SNR.
    }
    \label{fig:spec_eff}
\end{figure}
